Model architectures to extrapolate emotional expressions in DNN-based text-to-speech

This paper proposes architectures that facilitate the extrapolation of emotional expressions in deep neural network (DNN)-based text-to-speech (TTS). In this study, the meaning of "extrapolate emotional expressions" is to borrow emotional expressions from others, and the collection of emotional speech uttered by target speakers is unnecessary. Although a DNN has potential power to construct DNN-based TTS with emotional expressions and some DNN-based TTS systems have demonstrated satisfactory performances in the expression of the diversity of human speech, it is necessary and troublesome to collect emotional speech uttered by target speakers. To solve this issue, we propose architectures to separately train the speaker feature and the emotional feature and to synthesize speech with any combined quality of speakers and emotions. The architectures are parallel model (PM), serial model (SM), auxiliary input model (AIM), and hybrid models (PM&AIM and SM&AIM). These models are trained through emotional speech uttered by few speakers and neutral speech uttered by many speakers. Objective evaluations demonstrate that the performances in the open-emotion test provide insufficient information. They make a comparison with those in the closed-emotion test, but each speaker has their own manner of expressing emotion. However, subjective evaluation results indicate that the proposed models could convey emotional information to some extent. Notably, the PM can correctly convey sad and joyful emotions at a rate of >60%.

==> chapter/apalike.tex <==
% apalike.tex, version 0.99b (8-Dec-10), for btxmac 0.99i, BibTeX 0.99c,
% TeX 3.0 or later.
%
% Copyright (C) 1990, 1991, 1992, 2010 Oren Patashnik.
% Unlimited copying and redistribution of this file are permitted as long as
% it is unmodified.  Modifications (and redistribution of modified versions)
% are also permitted, but only if the resulting file is renamed.
%
% This file, apalike.tex, contains TeX macros that let you use the
% apalike bibliography style with plain TeX.  In essence, this file
% provides the TeX counterpart to apalike.sty, the LaTeX style file
% required for using the apalike bibliography style.  Please report any
% bugs (outright goofs, misfeatures, or unclear documentation) to
% biblio@tug.org.  These macros will become frozen
% shortly after BibTeX version 1.00 is released.
%
% AMS-TEX WARNING: This style (apalike) doesn't work with AmS-TeX's
% `amsppt' style, because AmS-TeX redefines the tie character `~' of
% plain TeX, and the `amsppt' style redefines plain TeX's `\nobreak'
% macro, so that a multiple-author reference for which `apalike'
% automatically produces an in-text citation like `(Jones et~al., 1992)'
% will throw AmS-TeX's `amsppt' style into an infinite loop, exceeding
% its input stack size.  (I've checked no other AmS-TeX styles for this
% problem.)  The AmS-TeX warning of btxmac.tex gives more information.
% END OF AMS-TEX WARNING.
%
% Editorial note (i.e., flame):
% Many journals require a style like `apalike', but I recommend that you
% not use it if you have a choice---use something like `plain' instead.
% Mary-Claire van Leunen (A Handbook for Scholars, Knopf, 1979) argues
% convincingly that a style like `plain' encourages better writing than
% one like `apalike'.  Furthermore the best argument for using an
% author-date style like `apalike'---that it's "the most practical"
% (The Chicago Manual of Style, University of Chicago Press, thirteenth
% edition, 1982, pages 400--401)---falls flat on its face with the new
% computer-typesetting technology.  For instance page 401 of the Chicago
% Manual anachronistically states "The chief disadvantage of [a style
% like `plain'] is that additions or deletions cannot be made after the
% manuscript is typed without changing numbers in both text references
% and list."  With (La)TeX the disadvantage obviously evaporates.
% Moreover, apalike indulges in what I think is a shortsighted practice:
% automatically abbreviating first names.  Abbreviating may occasionally
% make the work a page shorter, but at the cost of a less useful
% reference list; that's too high a cost for such a marginal benefit.
% The offense isn't egregious for a name like `Donald E. Knuth'---at
% least among those familiar with his field---since there aren't many
% other `D. E. Knuth's floating around.  But referring to `D. E. Smith'
% in a field having more than one can be quite confusing.  Moreover,
% with the proliferation of computers and citation indexes nowadays,
% it's important to indicate in the reference list an author's name
% exactly as it appears in the work cited.  Automatically abbreviating
% first names is simply bad scholarship.  (End of flame.)
%
% To use these macros you need the btxmac.tex macros, which let you use
% BibTeX with plain TeX (rather than with LaTeX); the file btxmac.tex
% explains those macros in detail, and gives examples.  You simply
% \input apalike right after you \input btxmac to invoke these macros.
%
%
%   HISTORY
%
% Oren Patashnik wrote the original version of these macros in December
% 1990, for use with btxmac.tex.
%
%   12-Dec-90  Version 0.99a, first general release.
%   29-Feb-92  0.99b, changed `\biblabelextrahang' to `\biblabelextraspace',
%                     to keep up with btxmac.tex version 0.99i.
%    8-Dec-10  Still version 0.99b, as the code itself was unchanged;
%                     this release clarified the license.
%
% Here, finally (I swear, I thought he was never gonna stop), are the
% macros.  The first bunch makes the label empty and sets 2em of
% hanging indentation (via \biblabelextraspace) for each entry.
%
\def\biblabelprint#1{\noindent}%
\def\biblabelcontents#1{}%
\def\bblhook{\biblabelextraspace = 2em }%
%
%
% And the last bunch formats an in-text citation: parens around the
% entire citation; semicolons separating individual references; and a
% comma between a reference and its note (like `page 41') if it exists.
%
\def\printcitestart{(}%         left paren
\def\printcitefinish{)}%        right parent
\def\printbetweencitations{; }% semicolon, space
\def\printcitenote#1{, #1}%     comma, space, note (if it exists)

